EVEREST: Efficient Masked Video Autoencoder by Removing Redundant Spatiotemporal Tokens

Masked Video Autoencoder (MVA) approaches have demonstrated their potential by significantly outperforming previous video representation learning methods. However, they waste an excessive amount of computations and memory in predicting uninformative tokens/frames due to random masking strategies. (e.g., over 16 nodes with 128 NVIDIA A100 GPUs). To resolve this issue, we exploit the unequal information density among the patches in videos and propose EVEREST, a surprisingly efficient MVA approach for video representation learning that finds tokens containing rich motion features and discards uninformative ones during both pre-training and fine-tuning. We further present an information-intensive frame selection strategy that allows the model to focus on informative and causal frames with minimal redundancy. Our method significantly reduces the computation and memory requirements of MVA, enabling the pre-training and fine-tuning on a single machine with 8 GPUs while achieving comparable performance to computation- and memory-heavy baselines on multiple benchmarks and the uncurated Ego4D dataset. We hope that our work contributes to reducing the barrier to further research on video understanding.

==> contents/fig_ssv2_time.tex <==
\begin{wrapfigure}{c}{0.49\linewidth}
    \small
    \centering
    % \vspace{-0.01in}
    \includegraphics[width=0.95\linewidth]{figures/images/ssv2_time.pdf}
\vspace{-0.1in}
     \caption{\small \textbf{Accuracy against training time} during pre-training and fine-tuning on \textbf{SSv2 dataset}~\cite{goyal2017something}. We used four NVIDIA GeForce RTX 3090 GPUs. In our model, we set $\rho_{pre}$ to 0.3 and 0.8 for pre-train and fine-tuning, respectively.}
    \label{fig:ssv2_time}
% \vspace{-0.2in}
\end{wrapfigure}


==> contents/fig_table.tex <==
\begin{figure*}
\vspace{-0.05in}
    \small
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{ccc}
    \includegraphics[width=0.32\linewidth]{figures/images/epochs_acc.pdf}&
     \includegraphics[width=0.32\linewidth]{figures/images/ptflops_ftflops.pdf}&
     \includegraphics[width=0.32\linewidth]{figures/images/}\\
     \textbf{(a) Training Results}&
     (b) GFLOPs both in pre-triaining and finetuning &
     (c) Ours\\
    \end{tabular}}
     \caption{\footnotesize {\textbf{Illustration of Motion-centric Token Selection.} (a) and (b) learn spatiotemporal representation by randomly masking the given video with a high ratio(e.g., 90\%) and reconstructing it(dashed lines cubes). However, different from the previous approaches we only reconstruct randomly selected partial tokens(marked as 'r' on the upper left) out of motion-activated tokens(visible tokens).}}
    \label{fig:concept}
\end{figure*}


==> contents/intro_concept_figure.tex <==
\begin{figure*}
% \vspace{-0.1in}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/images/wide_video.pdf}
% \vspace{-0.1in}
    \small
    \centering
    \resizebox{0.95\textwidth}{!}{%
    \begin{tabular}{cccc}
    \includegraphics[width=0.23\linewidth]{figures/images/masking_agnostic.pdf}&
     \includegraphics[width=0.23\linewidth]{figures/images/masking_tube.pdf}&
     \includegraphics[width=0.23\linewidth]{figures/images/masking_ours_final_2.pdf}&
     \includegraphics[width=0.23\linewidth]{figures/memory.pdf}\\
     \textbf{(a) Random}~\cite{feichtenhofer2022masked}&
     \textbf{(b) Space-only}~\cite{tong2022videomae}&
     \textbf{(c) MATS (Ours)}&
     \\
    \end{tabular}}
     \caption{\small{\textbf{Illustration of Motion-Aware Token Selection.} \textbf{(a-b)} MVM methods forward a few tokens in arriving video frames into the encoder based on fully random and time-only random selection, and then the decoder \emph{reconstructs entire tokens}. \textbf{(c)} Unlike prior works, our proposed motion-aware masking strategy only recovers key tokens related to moving objects (visible). To do this, we use encoder features extracted from randomly selected tokens among them (visible and colored).}}
    \label{fig:concept}
\vspace{-0.1in}
\end{figure*}


==> contents/method_illustration.tex <==
\begin{figure}
    \small
    \centering
    \includegraphics[width=0.95\linewidth]{figures/images/overview.pdf}
\vspace{-0.1in}
     \caption{\footnotesize {\textbf{Our proposed Motion-centric Token selection.} }}
    \label{fig:ours}
\end{figure}


==> contents/supplement_table_ablation_sampling.tex <==
\begin{wraptable}{r}{3.cm}
\centering
% \vspace{-0.1in}
%\addtolength{\tabcolsep}{-2.8pt}  
\caption{\small \bf Ablation study of motion-aware adaptive frame selection of MATS. }
\vspace{0.1in}
\resizebox{0.18\textwidth}{!}{
\renewcommand{\arraystretch}{1.0}
\renewcommand{\tabcolsep}{3pt}
\begin{tabular}{c c}
        \toprule
        \vspace{-0.02in}
        $\alpha$ & \textbf{Acc. (\%)} \\
        \midrule
        { -} & { 73.17}\\
        { 1.3} & { 73.54}\\
        \highlight{ 1.5} & { \textbf{73.85}}\\
        { 1.8} & { 73.79}\\
        { 2.0} & { 73.80}\\
\bottomrule
\end{tabular}}
\label{tab:ablation_sampling}
\end{wraptable}

==> contents/supplement_table_hyperparams_oscc.tex <==
\begin{table}[h]
\vspace{-0.15in}
\begin{minipage}{0.49\linewidth}
    \vspace{-0.1in}
    \input{contents/supplement_table_hyperparams_oscc_pt}
\end{minipage}
\hfill
\begin{minipage}{0.49\linewidth}
    \vspace{-0.1in}
    \input{contents/supplement_table_hyperparams_oscc_ft}
\end{minipage}
    \vspace{-0.05in}
    \caption{\small \textbf{Pre-training (Left) and Fine-tuning (Right) settings for OSCC.}}
    \label{tab:supplement_table_hyperparams_oscc}
    \vspace{-0.1in}
\end{table}

==> contents/supplement_table_hyperparams_oscc_ft.tex <==
\vspace{0.05in}
\centering
        \resizebox{1.0\textwidth}{!}{
\renewcommand{\arraystretch}{1.0}
\renewcommand{\tabcolsep}{9pt}
\begin{tabular}{c|c}
& {OSCC}\\
\midrule
optimizer&\\
base learning rate&\\
weight decay&\\
batch size&\\
\bottomrule
\end{tabular}}

==> contents/supplement_table_hyperparams_oscc_pt.tex <==
\vspace{0.05in}
\centering
        \resizebox{1.0\textwidth}{!}{
\renewcommand{\arraystretch}{1.0}
\renewcommand{\tabcolsep}{9pt}
\begin{tabular}{c|c}
& {OSCC}\\
\midrule
optimizer&\\
base learning rate&\\
weight decay&\\
batch size&\\
\bottomrule
\end{tabular}}

==> contents/supplement_vis_2.tex <==
\begin{figure*}[h]
    \centering
        \includegraphics[width=0.8\linewidth]{figures/images/supplement_5.pdf}
\vspace{-0.05in}
     \caption{\small {\textbf{More Examples of Motion-Aware Token selection.} We show the original video frames in the first row, Motion-Aware masking results in the second row, and obtained importance heatmaps in the last row on UCF101~\cite{soomro2012ucf101} dataset. $\rho_{pre}$ is set to 0.3 in this example.}}
    \label{fig:supple_visss_2}
\end{figure*}



==> contents/table_EVEREST-Finetuninig_with_other_MVAs.tex <==
% \begin{table*}[t!]
% \begin{minipage}{.48\linewidth}

%     \caption{\small \textbf{EVEREST-Finetuning with other MVAs on K400.} We apply our EVEREST for finetuning the pre-trained models~(ViT-B) by SoTA MVAs. We measure the memory usage with the same batch size of 128. While SoTA methods use full tokens during fine-tuning, our EVEREST uses only redundancy-robust tokens that \textbf{reduces significant computational cost and memory usage} with comparable accuracy.}
%     \vspace{-0.15in}
%     \center
%     \resizebox{0.9\linewidth}{!}{
%         \begin{tabular}{ccccc}
%         \hline
%         PT-Method & FT-Method       & GFLOPs & Memory  & Top-1         \\ \hline
%         VideoMAE  & Full-token      & 180.5  & 362.5 GB      & 81.5          \\
%         \cellcolor{gg}VideoMAE  & \cellcolor{gg}\textbf{EVEREST}   & \cellcolor{gg}98.1   & 1\cellcolor{gg}78.4 GB      & \cellcolor{gg}81.6          \\ \hline
%         MME       & Full-token      & 180.5  & 362.5 GB      & 81.8          \\
%         \cellcolor{gg}MME       & \cellcolor{gg}\textbf{EVEREST}   & \cellcolor{gg}98.1   & \cellcolor{gg}178.4 GB      & \cellcolor{gg}82.0          \\ \hline
%         MVD       & Full-token      & 180.5  & 362.5 GB      & 83.4          \\
%         \cellcolor{gg}MVD       & \cellcolor{gg}\textbf{EVEREST}   & \cellcolor{gg}98.1   & \cellcolor{gg}178.4 GB      & \cellcolor{gg}82.8          \\ \hline
%         \end{tabular}
%     }
%     \label{tab:ft_mem}
%   % \vspace{-0.4cm}
% \end{minipage}\hspace{0.15in}
% \begin{minipage}{.48\linewidth}
  
% \centering
%     \vspace{-0.05in}
%     \includegraphics[width=0.85\linewidth]{figures/images/ssv2.pdf}
%     \vspace{-0.1in}
%      \captionof{figure}{\small \textbf{Accuracy over training time} on SSv2. 4 NVIDIA RTX 3090 GPUs are used. We set $\rho_{pre}$ to 0.3 and 0.8 for pre-train and fine-tuning, respectively.}
%     \label{fig:ssv2_time}
%     % \vspace{-0.15in}
% \end{minipage}
% \end{table*}


==> contents/table_Pre-training_time_Memory_comparison.tex <==
% \begin{table}[t!]
%   \caption{\small \textbf{Pre-training time \& Memory comparison with SoTA MVAs on K400.} We measure the pre-training time for an epoch under a single-node machine equipped with 8$\times$A6000~(48GB) GPUs. We use ViT-B and a batch size of 128. Note that MME~\citep{sun2023mme} should pre-compute the optical flow for the entire video data before pre-training. We exclude the time and memory of MME for optical flow computations in the table.}
%   % \centering
%     % \begin{adjustbox}{width=\columnwidth, center}
%     \vspace{-0.15in}
%     \center
%     \resizebox{0.9\linewidth}{!}{
%         \begin{tabular}{lcc}
%         \hline
%         Method                 & PT-Time & Memory \\ \hline
%         VideoMAE~\citep{tong2022videomae}               & 18m   42s            & 150.3 GB              \\
%         MME~\citep{sun2023mme}                    & 10m   15s            & 121.2 GB              \\
%         MVD~\citep{wang2023mvd}                    & 51m   55s            & 274.9 GB              \\
%         \cellcolor{gg}\textbf{EVEREST   (ours)} & \cellcolor{gg}\textbf{8m   18s}    & \cellcolor{gg}~\textbf{66.3} GB      \\ \hline
%         \end{tabular}
%     }    
%   \label{tab:pt_mem}%
%   % \vspace{-0.1in}
% \end{table}


==> contents/table_ablations.tex <==
\begin{table}[t!]
\centering
\begin{minipage}{0.49\linewidth}
    % \includegraphics[width=0.95\linewidth]{figures/images/ssv2_time.pdf}
    \includegraphics[width=0.95\linewidth]{figures/images/ssv2.pdf}
    \vspace{-0.1in}
     \captionof{figure}{\small \textbf{Accuracy over training time} on SSv2. 4 NVIDIA RTX 3090 GPUs are used. We set $\rho_{pre}$ to 0.3 and 0.8 for pre-train and fine-tuning, respectively.}
    \label{fig:ssv2_time}
\end{minipage}
\hfill
% \hspace{0.2in}
\begin{minipage}{0.49\linewidth}
    \vspace{-0.1in}
    \caption{\small \textbf{Memory usage comparison} during the pre-training (one node, A100$\times$8 GPUs) on K400. The memory gaps grow up when increasing batch size and model size. Especially, our EVEREST with ViT-L achieves about $\mathbf{4\times}$ \textbf{better} efficiency than VideoMAE (634.1GB). \highlight{\emph{OOM}} indicates \textit{out-of-memory}.}
    \vspace{-0.1in}
    % \begin{adjustbox}{width=\columnwidth, center}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lccccc}
    \toprule
        \multirow{2}{*}{Method} & \multirow{2}{*}{Backbone} & \multicolumn{4}{c}{Effective Batch Size}\\
        && 128 & 256 & 512 & 1024\\
    \midrule
    \vspace{0.03in}
    &{ViT-S} & 71.9  & 117.4  & 233.6  & 443.6  \\ 
    \vspace{0.03in}
    VideoMAE&{ViT-B} & 258.4  & 486.4  & \highlight{\emph{OOM}} & \highlight{\emph{OOM}}\\
    \vspace{0.03in}
    &{ViT-L} & 353.9  & 634.1  & \highlight{\emph{OOM}} & \highlight{\emph{OOM}}\\
    \midrule
     \vspace{0.03in}
     &{ViT-S}& \textbf{31.9 } & \textbf{59.9 } & \textbf{95.6 } & \textbf{173.1 }\\
    \vspace{0.03in}
    Ours &{ViT-B}& \textbf{60.0 } & \textbf{91.2 } & \textbf{151.2 } & \textbf{273.6 }\\
    \vspace{0.03in}
    &{ViT-L}& \textbf{117.3 } & \textbf{164.1 } & \textbf{258.9 } & \textbf{428.4 }\\
    \bottomrule
    \end{tabular}}
    \vspace{-0.1in}
    % \end{adjustbox}
    \label{tab:mem-allocation2}
\end{minipage}
% \vspace{-0.15in}
\end{table} 


% \begin{table}[t!]
% \centering
% \begin{minipage}{0.49\linewidth}
%     \includegraphics[width=0.95\linewidth]{figures/images/ssv2_time.pdf}
%     \vspace{-0.1in}
%      \captionof{figure}{\small \textbf{Accuracy over training time} on SSv2. 4 NVIDIA RTX 3090 GPUs are used. We set $\rho_{pre}$ to 0.3 and 0.8 for pre-train and fine-tuning, respectively.}
%     \label{fig:ssv2_time}
% \end{minipage}
% \hfill
% % \hspace{0.2in}
% \begin{minipage}{0.49\linewidth}
%     % \begin{tabular}[t]
%     \vspace{-0.1in}
%     \caption{\small \textbf{Comparison with public SoTA methods for OSCC on Ego4D val set.} We set the sampling ratio $\alpha=1.5$ for EVEREST. ‘V’ and ‘T’ refer to \textit{visual} and \textit{text} for pre-trained data modalities from the OSCC.}
%     % \vspace{-0.1in}
%     \label{tab:table_oscc_results}
%     \begin{adjustbox}{width=0.95\linewidth, center}
%     \begin{tabular}{lcl}
%     \toprule
%     \vspace{0.03in}
%     Method         & Modality & Accuracy~(\%)      \\ \midrule
%     \vspace{0.03in}
%     Egocentric VLP~\citep{kevin2022egovlp} & V+T      & 73.9          \\ \midrule
%     \vspace{0.03in}
%     SViT~\citep{escobar2022video}           & V        & 69.8          \\
%     \vspace{0.03in}
%     TarHeels~\citep{islam2022object}       & V        & 70.8          \\
%     \textbf{EVEREST (Ours)} & V & {\textbf{76.2} \textbf{\footnotesize\highlight{(+5.4\%p)}}} \\ \bottomrule
%     \end{tabular}
%     \end{adjustbox}
%     % \vspace{0.05in}
%     % \end{tabular}
% \end{minipage}
% \vspace{-0.15in}
% \end{table} 




==> contents/table_batch_size.tex <==
\begin{table}[h]
\centering
% \vspace{-0.1in}
%\addtolength{\tabcolsep}{-2.8pt}  
\resizebox{0.47\textwidth}{!}{
\renewcommand{\arraystretch}{1.0}
\renewcommand{\tabcolsep}{3pt}
\begin{tabular}{lcccc}

\toprule
\multirow{2}{*}{\textbf{Method}}
&\multicolumn{2}{c}{\textbf{Pre-train}}&\multicolumn{2}{c}{\textbf{Fine-tune}}\\
&{\textbf{Batch size}}&{\textbf{GPU(G)}}&{\textbf{Batch size}}&{\textbf{GPU(G)}}\\
\midrule
{MAE~\cite{feichtenhofer2022masked}}&{16}&{23.2}&{4}&{20.3}\\
{VideoMAE$^\dagger$~\cite{tong2022videomae}}&{24}&{23.6}&{8}&{18.7}\\
\midrule
\multirow{4}{*}{\textbf{Ours}$^\dagger$}
&{16}&{7.2}&{4}&{6.5}\\
&{24}&{9.2}&{8}&{9.5}\\
&{36}&{12.1}&{12}&{14.0}\\
&{\textbf{72}}&{\textbf{20.6}}&{\textbf{16}}&{\textbf{17.1}}\\

% \hline \hline
\bottomrule
\end{tabular}}
\vspace{-0.1in}
\caption{\small GPU memory usage comparison of ViT-B between previous Masking-based Video models with respect to batch size.$^\dagger$ use Deepspeed frameworks during fine-tuning. These experiments are conducted on the same NVIDIA GeForce RTX 3090 GPU.}
\label{tab:batchsize}
% \vspace{-0.1in}
\end{table}

==> contents/table_comparison.tex <==
\begin{table}[t!]
\centering
\begin{minipage}{0.49\linewidth}
    \caption{\small \textbf{Performance comparison on
K400 and SSv2 datasets.}}
\begin{adjustbox}{width=\columnwidth, center}
\begin{tabular}{l c c c c c}
\toprule
    \multirow{2}{*}{Method} & \multirow{2}{*}{Backbone} & \multirow{2}{*}{Extra data} & \multirow{2}{*}{Frames} & \multicolumn{2}{c}{Top-1 Acc.(\%)}\\
    &&&&{\textbf{K400}}&{\textbf{SSv2}}\\
\midrule
    K-centered~\cite{Park_2022_ECCV}&{ViT-B~\cite{dosovitskiy2020image}}&{ImageNet-1K~\cite{ILSVRC15}}&{8} &{75.7} & {63.8}\\
    K-centered~\cite{Park_2022_ECCV}&{TimeSformer~\cite{bertasius2021timesformer}}&{ImageNet-1K~\cite{ILSVRC15}}&{8} &{78.0} & {63.8}\\
    K-centered~\cite{Park_2022_ECCV}&{Motionformer~\cite{patrick2021mformer}}&{ImageNet-1K~\cite{ILSVRC15}}&{8} &{74.9} & {62.2}\\
    K-centered~\cite{Park_2022_ECCV}&{XViT~\cite{bulat2021space}}&{ImageNet-1K~\cite{ILSVRC15}}&{8 / 16} &{73.1} & {62.8}\\
\midrule
    VideoMAE~\cite{tong2022videomae}&{ViT-S}&{\ding{55}}&{16} &{79.0} & {N/A}\\
    VideoMAE~\cite{tong2022videomae}&{ViT-B}&{\ding{55}}&{16} &{81.5} & {69.7}\\
    VideoMAE~\cite{tong2022videomae}&{ViT-L}&{\ding{55}}&{16} &{85.2} & {74.0}\\
\midrule
    \textbf{MATS (Ours)}&{ViT-S}&{\ding{55}}&{16}&{\TBD{78.6}} & {\TBD{00.0}}\\
    \textbf{MATS (Ours)}&{ViT-B}&{\ding{55}}&{16}&{\TBD{80.9}} & {\TBD{00.0}}\\
    \textbf{MATS (Ours)}&{ViT-L}&{\ding{55}}&{16}&{\TBD{83.1}} & {\TBD{00.0}}\\
\bottomrule
\end{tabular}
\end{adjustbox}
    \vspace{0.05in}
\end{minipage}
\hfill
\begin{minipage}{0.49\linewidth}
    \caption{\small \textbf{Performance comparison with strong baselines on
UCF101 and HMDB51 datasets} without using the pre-training step on a large-scale dataset. Several results are drawn from \cite{diba2021vi2clr} and \cite{tong2022videomae}.}
\begin{adjustbox}{width=\columnwidth, center}
\begin{tabular}{l c c c c c}
\toprule
    \multirow{2}{*}{Method} & \multirow{2}{*}{Backbone} & \multirow{2}{*}{Extra data} & \multirow{2}{*}{Frames} & \multicolumn{2}{c}{Top-1 Acc.(\%)}\\
    &&&&{\textbf{UCF101}}&{\textbf{HMDB51}}\\
\midrule
    % OPN \cite{lee2017unsupervised}& {VGG} & {UCF101} & {N/A} & {59.6} & {23.8}\\
    VCOP~\cite{xu2019self}& {R(2+1)D} & {UCF101} & {N/A} & {72.4} & {30.9}\\
    CoCLR~\cite{han2020self}& {S3D-G} & {UCF101} & {32} & {81.4} & {52.1}\\
    Vi$^{2}$~CLR\cite{diba2021vi2clr}& {S3D} & {UCF101} & {32} & {82.8} & {52.9}\\
    CoCLR~\cite{han2020self}& {S3D-G} & {K400} & {32} & {87.9} & {54.6}\\
    Vi$^{2}$~CLR\cite{diba2021vi2clr}& {S3D} & {K400} & {32} & {89.1} & {55.7}\\
    RSPNet~\cite{chen2021rspnet}& {S3D-G} & {K400} & {64} & {93.7} & {64.7}\\    
    % $\rho\text{SimCLR}_{\rho=2}${\scriptsize \cite{feichtenhofer2021large}}& {SlowOnly-R50} & {K400} & {8} & {88.9} & {N/A} \\    
    $\rho\text{SwAV}_{\rho=2}$~{\cite{feichtenhofer2021large}}& {SlowOnly-R50} & {K400} & {8} & {87.3} & {N/A}\\
    $\rho\text{MoCo}_{\rho=2}$~{\cite{feichtenhofer2021large}}& {SlowOnly-R50} & {K400} & {8} & {91.0} & {N/A}\\
    $\rho\text{BYOL}_{\rho=2}$~{\cite{feichtenhofer2021large}}& {SlowOnly-R50} & {K400} & {8} & {92.7} & {N/A}\\
\midrule    
    VideoMAE~\cite{tong2022videomae}&{ViT-B}&{\ding{55}}&{16} &{91.3} & {62.6}\\
\midrule
    \textbf{MATS (Ours)}&{ViT-B}&{\ding{55}}&{16}&{93.4} & {68.1}\\
\bottomrule
\end{tabular}
\end{adjustbox}
    \vspace{0.05in}
\end{minipage}
\end{table} 

==> contents/table_example.tex <==
% \begin{table*}[t!]
% \tiny
% \begin{center}
% \caption{\small Performance comparison of OCS and other baselines on balanced and imbalanced continual learning. We report the mean and standard-deviation of the average accuracy (Accuracy) and average forgetting (Forgetting) across five independent runs. The best results are highlighted in {\bf bold}.}
% \vspace{-0.1in}
% \resizebox{\textwidth}{!}{%
% \addtolength{\tabcolsep}{-2.8pt}  
% \begin{tabular}{llc cccc  ccc}
% % \hline 
% % \hline 
% \toprule
% % & {}&\multicolumn{2}{c}{\textbf{Rotated MNIST}} &\multicolumn{2}{c}{\textbf{Split CIFAR-100}}&\multicolumn{2}{c}{\textbf{Multiple Datasets}} \\
% % \hline  \\
% %\midrule
% & \textbf{Pre-training} & \textbf{Downstream Task} & \textbf{Fine-tuning (end-to-end)} & \textbf{ViT-B} & \textbf{ViT-L} & \textbf{ViT-H} \\
% \midrule
% \parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{MAE}}}
% & ImageNet1K & 
% {Semantic Segmentation (mIoU) } & {ADE20K (\checkmark)} & 
% {\scriptsize 48.1} & {\scriptsize 53.6} & 
% {-} \\
 
% & ImageNet1K &
% {Image Classification (Acc) } & {iNat 2017 (\checkmark)}  & 
% {\scriptsize 70.5} & {\scriptsize 75.7} & 
% {\scriptsize 79.3} \\
 
% & ImageNet1K &
% {Image Classification (Acc) } & {iNat 2018 (\checkmark)}  & 
% {\scriptsize 75.4} & {\scriptsize 80.1} & 
% {\scriptsize 83.0} \\
 
% & ImageNet1K &
% {Image Classification (Acc) } & {iNat 2019 (\checkmark)}  & 
% {\scriptsize 80.5} & {\scriptsize 83.4} & 
% {\scriptsize 85.7} \\
 
% & ImageNet1K &
% {Image Classification (Acc) } & {Places205 (\checkmark)}  & 
% {\scriptsize 63.9} & {\scriptsize 65.8} & 
% {\scriptsize 65.9} \\
 
% & ImageNet1K &
% {Image Classification (Acc) } & {Places365 (\checkmark)}  & 
% {\scriptsize 57.9} & {\scriptsize 59.4} & 
% {\scriptsize 59.8} \\

% & ImageNet1K &
% {Object Detection ($\text{AP}^{\text{box}}$) } & {COCO (\checkmark)} & 
% {\scriptsize 50.3} & {\scriptsize 53.3} & 
% {-} \\

% \midrule
% % & {}&\multicolumn{2}{c}{\textbf{Rotated MNIST}} &\multicolumn{2}{c}{\textbf{Split CIFAR-100}}&\multicolumn{2}{c}{\textbf{Multiple Datasets}} \\
% % \hline  \\
% %\midrule
% & \textbf{Pre-training} & \textbf{Downstream Task} & \textbf{Fine-tuning (end-to-end)} & \textbf{ResNet-18} & \textbf{ResNet-50} \\

% \midrule

% \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{VFS}}}
% & Kinetics & 
% {Video Object Segmentation ($\mathcal{J}$\&$\mathcal{F_{\textit{m}}}$)} & {DAVIS-2017} & 
% {\scriptsize 66.7} & {\scriptsize 68.9}\\

% & Kinetics  & 
% {Human Pose Tracking (PCK@0.1) } & {JHMDB} & 
% {\scriptsize 60.5} & {\scriptsize 60.9}\\

% & Kinetics & 
% {Human Part Tracking (mIoU) } & {VIP} & 
% {\scriptsize 39.9} & {\scriptsize 43.2}\\

% & Kinetics & 
% {Visual Object Tracking (Precision) } & {OTB-100} & 
% {\scriptsize 68.9} & {\scriptsize 73.9}\\


% % \hline \hline
% \bottomrule
% \end{tabular}}
% \label{tab:main_table}
% \vspace{-0.25in}
% \end{center}
% \end{table*}

==> contents/table_ft_comparison.tex <==
\begin{table}[t]
  \small
  \centering
\caption{\small \textbf{EVEREST-Finetuning with other pre-trained models.} We apply our EVEREST for finetuning the pre-trained models~(ViT-B) by SoTA MVMs. Note that since VideoMAE, MME, and MVD use different batch sizes, we measured the memory usage of all models with the same batch size of 128. While SoTA methods use full-tokens during finetuning, our EVEREST uses only selected tokens and in turn \textbf{reduces significant computation cost and memory usage} with comparable accuracy.}
\begin{tabular}{lcccc}
\hline
PT-Method & FT-Method       & GFLOPs & Memory usage  & Top-1         \\ \hline
VideoMAE  & Full-token      & 180.5  & 362.5 GB      & 81.5          \\
VideoMAE  & \textbf{EVEREST}   & 98.1   & 178.4 GB      & 81.6          \\ \hline
MME       & Full-token      & 180.5  & 362.5 GB      & 81.8          \\
MME       & \textbf{EVEREST}   & 98.1   & 178.4 GB      & 82.0          \\ \hline
MVD       & Full-token      & 180.5  & 362.5 GB      & 83.4          \\
MVD       & \textbf{EVEREST}   & 98.1   & 178.4 GB      & 82.8          \\ \hline
\end{tabular}
\end{table}


==> contents/table_k400_ssv2.tex <==
\begin{table}[t!]
% \vspace{0.05in}
\centering
\caption{\small \textbf{Performance comparison on
K400 and SSv2 datasets.}}
% \begin{adjustbox}{width=\columnwidth, center}
\resizebox{0.7\columnwidth}{!}{
\begin{tabular}{l c c c c c}
\toprule
    \multirow{2}{*}{Method} & \multirow{2}{*}{Backbone} & \multirow{2}{*}{Extra data} & \multirow{2}{*}{Frames} & \multicolumn{2}{c}{Top-1 Acc.(\%)}\\
    &&&&{\textbf{K400}}&{\textbf{SSv2}}\\
\midrule
    K-centered~\cite{Park_2022_ECCV}&{ViT-B~\cite{dosovitskiy2020image}}&{IN-1K}&{8} &{75.7} & {63.8}\\
    K-centered~\cite{Park_2022_ECCV}&{TimeSformer~\cite{bertasius2021timesformer}}&{IN-1K}&{8} &{78.0} & {63.8}\\
    K-centered~\cite{Park_2022_ECCV}&{Motionformer~\cite{patrick2021mformer}}&{IN-1K}&{8} &{74.9} & {62.2}\\
    K-centered~\cite{Park_2022_ECCV}&{XViT~\cite{bulat2021space}}&{IN-1K}&{8 / 16} &{73.1} & {62.8}\\
\midrule
    VideoMAE~\cite{tong2022videomae}&{ViT-S}&{\ding{55}}&{16} &{79.0} & {N/A}\\
    VideoMAE~\cite{tong2022videomae}&{ViT-B}&{\ding{55}}&{16} &{81.5} & {69.7}\\
    VideoMAE~\cite{tong2022videomae}&{ViT-L}&{\ding{55}}&{16} &{85.2} & {74.0}\\
\midrule
    \textbf{MATS (Ours)}&{ViT-S}&{\ding{55}}&{16}&{\TBD{78.6}} & {\TBD{00.0}}\\
    \textbf{MATS (Ours)}&{ViT-B}&{\ding{55}}&{16}&{\TBD{80.9}} & {\TBD{00.0}}\\
    \textbf{MATS (Ours)}&{ViT-L}&{\ding{55}}&{16}&{\TBD{83.1}} & {\TBD{00.0}}\\
\bottomrule
\end{tabular}
}
% \end{adjustbox}
\label{tab:k400&ssv2}
% \vspace{-0.15in}
\end{table}

==> contents/table_main.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[t]
  \centering
  \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{lcccccrcccc}
    \toprule
    \multirow{2}[4]{*}{Method} & \multirow{2}[4]{*}{Backbone} & \multirow{2}[4]{*}{Extra data} & \multirow{2}[4]{*}{Label} & \multirow{2}[4]{*}{Frames} & \multirow{2}[4]{*}{GFLOPs} & \multirow{2}[4]{*}{Param.} & \multicolumn{2}{c}{Kinetics-400} & \multicolumn{2}{c}{SSv2} \\
\cmidrule{8-11}          &       &       &       &       &       &       & top-1 & top-5 & top-1 & top-5 \\
    \midrule
    TimeSformer~\cite{bertasius2021timesformer} & ViT-B & IN-21K & \checkmark     & 8     & $196\times1\times3$ & 121M  & 78.3  & 93.7  & 59.1  & 85.6 \\
    Motionformer~\cite{patrick2021mformer} & ViT-B & IN-21K & \checkmark     & 16    & $370\times10\times3$ & 121M  & 79.7  & 94.2  & 66.5  & 90.1 \\
    VideoSwin~\cite{liu2022videoswin}  & Swin-B & IN-21K & \checkmark  & 32 & $282\times4\times3$ & 88M   & 80.6  & 94.6  & 69.6  & 92.7 \\
    BEVT~\cite{wang2022bevt}  & Swin-B & IN-1K+DALLE & \ding{55}  & 32 & $282\times4\times3$ & 88M   & 80.6  & N/A  & 70.6  & N/A \\
    SVT~\cite{ranasinghe2022svt}   & ViT-B & IN-21K &  \ding{55}    & 8+64  & $196\times1\times3$ & 87M   & 78.1  & N/A     & 59.2  & N/A \\
    \midrule
    VideoMAE~\cite{tong2022videomae} & ViT-B & \ding{55}     & \ding{55}     & 16    & $180\times5\times3$ & 87M   & 80.9  & 94.7  & 69.3  & 92.3 \\
    MAE~\cite{feichtenhofer2022masked}   & ViT-B & \ding{55}     & \ding{55}     & 16    & $180\times7\times3$ & 87M   & 81.3  & 94.9  & N/A     & N/A \\
    \midrule
    \textbf{VideoMS (Ours)}  & ViT-B & \ding{55}     & \ding{55}     & 16    &  $98\times5\times3$    & 87M   & -     & -     & -     & - \\
    \bottomrule
    \end{tabular}%
    \end{adjustbox}
    \caption{\small \textbf{Comparison to state-of-the-art methods on Kinetics-400 and SSv2.} VideoMAE is trained for 800 epoch. VideoSwin for SSv2 is pre-trained on IN-21K+K400.}
  \label{tab:main_previous}%
  \vspace{-0.15in}
\end{table*}%




% \begin{table*}
% \centering
% \caption{\small ViT-B performance comparison of \textbf{Ours} and other masking baselines on large-scale datasets. We report the number of forwarded embedded vectors per given video and GFLOPs during pre-training(encoder and decoder) and fine-tuning, respectively, and show the efficiency and effectiveness of our token selection on each dataset. The best results are highlighted in {\bf bold}.}

% \vspace{-0.1in}
% %\addtolength{\tabcolsep}{-2.8pt}  
% \resizebox{1.0\textwidth}{!}{
% \renewcommand{\arraystretch}{1.0}
% \renewcommand{\tabcolsep}{9pt}
% \begin{tabular}{cccccccccc}

% \toprule
% \multirow{2}{*}{\textbf{Masking}} & &\textbf{Pre-train}&& \multicolumn{2}{c}{\textbf{Fine-tune}} & \multicolumn{2}{c}{ \textbf{Kinetics-400}} &  \multicolumn{2}{c}{ \textbf{SSv2}} \\
% % \cmidrule(l{2pt}r{2pt}){5-6}
% % \cmidrule(l{2pt}r{2pt}){7-8}
% & \textbf{\# enc.}&\textbf{\# dec.} &\textbf{GFLOPs} &\textbf{\# vec.} &\textbf{GFLOPs}&\textbf{top-1} & \textbf{top-5} & \textbf{top-1} & \textbf{top-5} \\
% \midrule
% TimeSformer~\cite{bertasius2021timesformer} & 
% {-} & 
% {-} & {-} &{-}&{$196\times1\times3$}&{77.9} & 
% {93.2} & {59.1} & 
% {85.6} \\
% Mformer~\cite{patrick2021mformer} & 
% {-} & 
% {-} & {-} &{-}&{$369.5\times3\times10$}&{79.7} & 
% {94.2} & {66.5} & 
% {90.1} \\
% SVT~\cite{ranasinghe2022svt} & 
% {-} & 
% {-} & {-} &{-}&{$196\times1\times3$}&{78.1} & 
% {-} & {59.2} & 
% {-} \\
% Agnostics~\cite{feichtenhofer2022masked} & 
% {157} & 
% {1569} & {46.1} &{1569}&{180.6}&{80.6} & 
% {90.6} & {69.6} & 
% {85.6} \\
% Agnostics~\cite{feichtenhofer2022masked} & 
% {157} & 
% {1569} & {46.1} &{1569}&{180.6}&{80.6} & 
% {90.6} & {69.6} & 
% {85.6} \\
% Agnostics~\cite{feichtenhofer2022masked} & 
% {157} & 
% {1569} & {46.1} &{1569}&{180.6}&{80.6} & 
% {90.6} & {69.6} & 
% {85.6} \\
% Agnostics~\cite{feichtenhofer2022masked} & 
% {157} & 
% {1569} & {46.1} &{1569}&{180.6}&{80.6} & 
% {90.6} & {69.6} & 
% {85.6} \\
 
% Tube~\cite{tong2022videomae} &
% {160} & 
% {1568} & {35.5} &{1568}&{180.5}&{80.5} & {90.7} & {68.6} & 
% {84.6} \\
 
% \textbf{Ours} & {156} & 
% {470} & {\textbf{22.7}} &{940}&{\textbf{98.1}}&{\textbf{81.5}} & {\textbf{91.6}} & {\textbf{71.6}} & 
% {\textbf{88.6}} \\

% % \hline \hline
% \bottomrule
% \end{tabular}}
% \label{tab:table1}
% \vspace{-0.1in}
% \end{table*}

% \begin{table*}
% \centering
% \caption{\small ViT-B performance comparison of \textbf{Ours} and other masking baselines on large-scale datasets. We report the number of forwarded embedded vectors per given video and GFLOPs during pre-training(encoder and decoder) and fine-tuning, respectively, and show the efficiency and effectiveness of our token selection on each dataset. The best results are highlighted in {\bf bold}.}

% \vspace{-0.1in}
% %\addtolength{\tabcolsep}{-2.8pt}  
% \resizebox{1.0\textwidth}{!}{
% \renewcommand{\arraystretch}{1.0}
% \renewcommand{\tabcolsep}{9pt}
% \begin{tabular}{cccccccccc}

% \toprule
% \multirow{2}{*}{\textbf{Masking} (ratio)} & &\textbf{Pre-train}&& \multicolumn{2}{c}{\textbf{Fine-tune}} & \multicolumn{2}{c}{ \textbf{Kinetics-400}} &  \multicolumn{2}{c}{ \textbf{SSv2}} \\
% % \cmidrule(l{2pt}r{2pt}){5-6}
% % \cmidrule(l{2pt}r{2pt}){7-8}
% & \textbf{\# enc.}&\textbf{\# dec.} &\textbf{GFLOPs} &\textbf{\# vec.} &\textbf{GFLOPs}&\textbf{top-1} & \textbf{top-5} & \textbf{top-1} & \textbf{top-5} \\
% \midrule
% Agnostics~\cite{feichtenhofer2022masked} (90\%) & 
% {157} & 
% {1569} & {46.1} &{1569}&{180.6}&{80.6} & 
% {90.6} & {69.6} & 
% {85.6} \\
% Agnostics~\cite{feichtenhofer2022masked} (90\%) & 
% {157} & 
% {1569} & {46.1} &{1569}&{180.6}&{80.6} & 
% {90.6} & {69.6} & 
% {85.6} \\
% Agnostics~\cite{feichtenhofer2022masked} (90\%) & 
% {157} & 
% {1569} & {46.1} &{1569}&{180.6}&{80.6} & 
% {90.6} & {69.6} & 
% {85.6} \\
% Agnostics~\cite{feichtenhofer2022masked} (90\%) & 
% {157} & 
% {1569} & {46.1} &{1569}&{180.6}&{80.6} & 
% {90.6} & {69.6} & 
% {85.6} \\
% Agnostics~\cite{feichtenhofer2022masked} (90\%) & 
% {157} & 
% {1569} & {46.1} &{1569}&{180.6}&{80.6} & 
% {90.6} & {69.6} & 
% {85.6} \\
% Agnostics~\cite{feichtenhofer2022masked} (90\%) & 
% {157} & 
% {1569} & {46.1} &{1569}&{180.6}&{80.6} & 
% {90.6} & {69.6} & 
% {85.6} \\
% Agnostics~\cite{feichtenhofer2022masked} (90\%) & 
% {157} & 
% {1569} & {46.1} &{1569}&{180.6}&{80.6} & 
% {90.6} & {69.6} & 
% {85.6} \\
 
% Tube~\cite{tong2022videomae} (90\%) &
% {160} & 
% {1568} & {35.5} &{1568}&{180.5}&{80.5} & {90.7} & {68.6} & 
% {84.6} \\
 
% \textbf{Ours (70\% → 90\%, 40\%)} & {156} & 
% {470} & {\textbf{22.7}} &{940}&{\textbf{98.1}}&{\textbf{81.5}} & {\textbf{91.6}} & {\textbf{71.6}} & 
% {\textbf{88.6}} \\

% % \hline \hline
% \bottomrule
% \end{tabular}}
% \label{tab:table1}
% \vspace{-0.1in}
% \end{table*}



==> contents/table_main_2.tex <==
\centering
\resizebox{1.0\textwidth}{!}{
        \renewcommand{\arraystretch}{0.95}
        \renewcommand{\tabcolsep}{2pt}
        \begin{tabular}{lcccccrcc}
    \toprule
    \multirow{2}[4]{*}{Method} & \multirow{2}[4]{*}{Backbone} & \multirow{2}[4]{*}{Extra data} & \multirow{2}[4]{*}{Label} & \multirow{2}[4]{*}{Frames} & \multirow{2}[4]{*}{GFLOPs} & \multirow{2}[4]{*}{Param.} & \multicolumn{2}{c}{Kinetics-400} \\
\cmidrule{8-9}          &       &       &       &       &       &       & top-1 & top-5 \\
    \midrule
    TimeSformer~\cite{bertasius2021timesformer} & ViT-B & IN-21K & \checkmark     & 8     & $196\times1\times3$ & 121M  & 78.3  & 93.7  \\
    Motionformer~\cite{patrick2021mformer} & ViT-B & IN-21K & \checkmark     & 16    & $370\times10\times3$ & 121M  & 79.7  & 94.2  \\
    VideoSwin~\cite{liu2022videoswin}  & Swin-B & IN-21K & \checkmark  & 32 & $282\times4\times3$ & 88M   & 80.6  & 94.6  \\
    BEVT~\cite{wang2022bevt}  & Swin-B & IN-1K+DALLE & \ding{55}  & 32 & $282\times4\times3$ & 88M   & 80.6  & N/A   \\
    SVT~\cite{ranasinghe2022svt}   & ViT-B & IN-21K &  \ding{55}    & 8+64  & $196\times1\times3$ & 87M   & 78.1  & N/A \\
    \midrule
    VideoMAE~\cite{tong2022videomae} & ViT-B & \ding{55}     & \ding{55}     & 16    & $180\times5\times3$ & 87M   & 80.9  & 94.7   \\
    MAE~\cite{feichtenhofer2022masked}   & ViT-B & \ding{55}     & \ding{55}     & 16    & $180\times7\times3$ & 87M   & 81.3  & 94.9   \\
    \midrule
    \textbf{Ours}  & ViT-B & \ding{55}     & \ding{55}     & 16    &  $98\times5\times3$    & 87M   & -     & - \\
    \bottomrule
\end{tabular}}
% \centering
% \resizebox{1.0\textwidth}{!}{
%         \renewcommand{\arraystretch}{0.95}
%         \renewcommand{\tabcolsep}{2pt}
%         \begin{tabular}{lcccccrcccc}
%     \toprule
%     \multirow{2}[4]{*}{Method} & \multirow{2}[4]{*}{Backbone} & \multirow{2}[4]{*}{Extra data} & \multirow{2}[4]{*}{Label} & \multirow{2}[4]{*}{Frames} & \multirow{2}[4]{*}{GFLOPs} & \multirow{2}[4]{*}{Param.} & \multicolumn{2}{c}{Kinetics-400} & \multicolumn{2}{c}{SSv2} \\
% \cmidrule{8-11}          &       &       &       &       &       &       & top-1 & top-5 & top-1 & top-5 \\
%     \midrule
%     TimeSformer~\cite{bertasius2021timesformer} & ViT-B & IN-21K & \checkmark     & 8     & $196\times1\times3$ & 121M  & 78.3  & 93.7  & 59.1  & 85.6 \\
%     Motionformer~\cite{patrick2021mformer} & ViT-B & IN-21K & \checkmark     & 16    & $370\times10\times3$ & 121M  & 79.7  & 94.2  & 66.5  & 90.1 \\
%     VideoSwin~\cite{liu2022videoswin}  & Swin-B & IN-21K & \checkmark  & 32 & $282\times4\times3$ & 88M   & 80.6  & 94.6  & 69.6  & 92.7 \\
%     BEVT~\cite{wang2022bevt}  & Swin-B & IN-1K+DALLE & \ding{55}  & 32 & $282\times4\times3$ & 88M   & 80.6  & N/A  & 70.6  & N/A \\
%     SVT~\cite{ranasinghe2022svt}   & ViT-B & IN-21K &  \ding{55}    & 8+64  & $196\times1\times3$ & 87M   & 78.1  & N/A     & 59.2  & N/A \\
%     \midrule
%     VideoMAE~\cite{tong2022videomae} & ViT-B & \ding{55}     & \ding{55}     & 16    & $180\times5\times3$ & 87M   & 80.9  & 94.7  & 69.3  & 92.3 \\
%     MAE~\cite{feichtenhofer2022masked}   & ViT-B & \ding{55}     & \ding{55}     & 16    & $180\times7\times3$ & 87M   & 81.3  & 94.9  & N/A     & N/A \\
%     \midrule
%     \textbf{Ours}  & ViT-B & \ding{55}     & \ding{55}     & 16    &  $98\times5\times3$    & 87M   & -     & -     & -     & - \\
%     \bottomrule
% \end{tabular}}

==> contents/table_main_integrated.tex <==
\begin{table}[t!]
\centering
\begin{minipage}{0.49\linewidth}
\caption{\small \textbf{Performance comparison with strong baselines on
UCF101, HMDB51, and SSv2 datasets} without using the pre-training step on a large-scale dataset. Several results are drawn from \cite{diba2021vi2clr} and \cite{tong2022videomae}. \textit{SR50} indicates \textit{SlowOnly-R50}.}
\vspace{0.05in}
\resizebox{\columnwidth}{!}{
    % \renewcommand{\arraystretch}{1.0}
    % \renewcommand{\tabcolsep}{3pt}
\begin{tabular}{l c c c c c}
\toprule
    \multirow{2}{*}{Method} & \multirow{2}{*}{Backbone} & \multirow{2}{*}{Extra data} & \multicolumn{3}{c}{T1 Acc~(\%)}\\
    &&&{\textbf{UCF101}}&{\textbf{HMDB51}}&{\textbf{SSv2}}\\
\midrule
    % OPN \citep{lee2017unsupervised}& {VGG} & {UCF101} & {N/A} & {59.6} & {23.8}\\
    VCOP~\citep{xu2019self}& {R(2+1)D} & {UCF101} & {72.4} & {30.9} & {N/A}\\
    CoCLR~\citep{han2020self}& {S3D-G} & {UCF101} & {81.4} & {52.1} & {N/A}\\
    Vi$^{2}$~CLR\citep{diba2021vi2clr}& {S3D} & {UCF101} & {82.8} & {52.9} & {N/A}\\
    CoCLR~\citep{han2020self}& {S3D-G} & {K400} & {87.9} & {54.6} & {N/A}\\
    Vi$^{2}$~CLR\citep{diba2021vi2clr}& {S3D} & {K400} & {89.1} & {55.7} & {N/A}\\
    RSPNet~\citep{chen2021rspnet}& {S3D-G} & {K400} & {93.7} & {64.7} & {55.0}\\    
    % $\rho\text{SimCLR}_{\rho=2}${\scriptsize \citep{feichtenhofer2021large}}& {SR50} & {K400} & {8} & {88.9} & {N/A} \\    
    % $\rho\text{SwAV}_{\rho=2}$~{\citep{feichtenhofer2021large}}& {SR50} & {K400}  & {87.3} &{N/A} &${51.7}_{(\rho=3)}$\\
    % $\rho\text{MoCo}_{\rho=2}$~{\citep{feichtenhofer2021large}}& {SR50} & {K400}  & {91.0} &{N/A} &${54.4}_{(\rho=3)}$\\
    % $\rho\text{BYOL}_{\rho=2}$~{\citep{feichtenhofer2021large}}& {SR50} & {K400}  & {92.7} &{N/A} &${55.8}_{(\rho=3)}$\\
    $\rho\text{SwAV}_{\rho=2}$~{\citep{feichtenhofer2021large}}& {SR50} & {K400}  & {87.3} &{N/A} &${51.7}$\\
    $\rho\text{MoCo}_{\rho=2}$~{\citep{feichtenhofer2021large}}& {SR50} & {K400}  & {91.0} &{N/A} &${54.4}$\\
    $\rho\text{BYOL}_{\rho=2}$~{\citep{feichtenhofer2021large}}& {SR50} & {K400}  & {92.7} &{N/A} &${55.8}$\\
% \midrule    
    VideoMAE~\citep{tong2022videomae}&{ViT-B}&{\ding{55}} &{91.3} & {62.6} & {64.3}\\
\midrule
    \cellcolor{gg}\textbf{EVEREST (Ours)}&\cellcolor{gg}{ViT-B}&\cellcolor{gg}{\ding{55}}& \cellcolor{gg}\textbf{93.4} & \cellcolor{gg}\textbf{68.1} & \cellcolor{gg}\textbf{64.6}\\
\bottomrule
\end{tabular}}
\label{tab:ucf&hmdb}
\end{minipage}
\hfill
\begin{minipage}{0.49\linewidth}
\centering
    \includegraphics[width=0.98\linewidth]{figures/images/merge_fig_3.pdf}
    \vspace{-0.1in}
    \captionof{figure}{\small \textbf{Performance \& GFLOPs Comparison} on UCF101 dataset. \textbf{(Left)} EVEREST outperforms VideoMAE for both masking ratios (75\% and 90\%) even at significantly fewer training epochs. %We additionally report the results of VideoMAE with a lower masking ratio (75\%) during pre-training. 
    \textbf{(Right)} Our EVEREST reduces GFLOPs during pre-training and fine-tuning compared to VideoMAE and ST-MAE.}
    \label{fig:a}
    % \end{figure}
\end{minipage} 
\vspace{-0.2in}
\end{table} 


% \begin{minipage}{0.49\linewidth}
% \centering
% \caption{\small \textbf{Performance comparison on
% K400 and SSv2 datasets.}}
% % \begin{adjustbox}{width=\columnwidth, center}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{l c c c c}
% \toprule
%     \multirow{2}{*}{Method} & \multirow{2}{*}{Backbone} & \multirow{2}{*}{Extra data} & {T1 Acc}\\
%     &&&{\textbf{K400}}\\
% \midrule
%     K-centered~\citep{Park_2022_ECCV}&{ViT-B~\citep{dosovitskiy2020image}}&{IN-1K}&{75.7} \\
%     K-centered~\citep{Park_2022_ECCV}&{TSformer~\citep{bertasius2021timesformer}}&{IN-1K} &{78.0} \\
%     K-centered~\citep{Park_2022_ECCV}&{Mformer~\citep{patrick2021mformer}}&{IN-1K} &{74.9} \\
%     K-centered~\citep{Park_2022_ECCV}&{XViT~\citep{bulat2021space}}&{IN-1K}&{73.1} \\
% \midrule
%     VideoMAE~\citep{tong2022videomae}&{ViT-S}&{\ding{55}}&{79.0}\\
%     VideoMAE~\citep{tong2022videomae}&{ViT-B}&{\ding{55}}&{81.5} \\
%     VideoMAE~\citep{tong2022videomae}&{ViT-L}&{\ding{55}}&{85.2} \\
% \midrule
%     \textbf{EVEREST (Ours)}&{ViT-S}&{\ding{55}}&{\TBD{78.6}} \\
%     \textbf{EVEREST (Ours)}&{ViT-B}&{\ding{55}}&{\TBD{80.9}} \\
%     \textbf{EVEREST (Ours)}&{ViT-L}&{\ding{55}}&{\TBD{83.1}} \\
% \bottomrule
% \end{tabular}
% }
% % \end{adjustbox}
% \label{tab:k400&ssv2}
% \end{minipage}

==> contents/table_main_test.tex <==
\begin{table*}[h]
\begin{minipage}{0.67\linewidth}
    \vspace{-0.1in}
    \input{contents/table_main_2}
\end{minipage}
\begin{minipage}{0.31\linewidth}
    \vspace{-0.1in}
    \input{contents/table_small_dataset}
\end{minipage}
    \vspace{-0.05in}
    \caption{\small \textbf{Comparison to state-of-the-art methods on large-scale datasets (left) and small-scale datasets (right).} (Left) VideoMAE is trained for 800 epoch. VideoSwin for SSv2 is pre-trained on IN-21K+K400. (Right) }
    \label{tab:main}
    \vspace{-0.1in}
\end{table*} 

==> contents/table_main_test_2.tex <==
\begin{table*}[h]
\begin{minipage}{0.67\linewidth}
    \vspace{-0.1in}
    \input{contents/table_main_2}
\end{minipage}
\begin{minipage}{0.31\linewidth}
    \vspace{-0.1in}
    \input{contents/table_small_dataset}
\end{minipage}
    \vspace{-0.05in}
    \caption{\small \textbf{Comparison to state-of-the-art methods on large-scale datasets (left) and small-scale datasets (right).} (Left) VideoMAE is trained for 800 epoch. VideoSwin for SSv2 is pre-trained on IN-21K+K400. (Right) }
    \label{tab:main_2}
    \vspace{-0.1in}
\end{table*} 

==> contents/table_mask_method_comparison.tex <==
\begin{table}[t!]
  \small
  \centering
\caption{\small \textbf{Masking strategy comparison.} To compare with EVEREST, we conduct experiments adopting a frame-wise masking strategy with 400 and 100 pre-training epochs and 100 and 10 fine-tuning epochs on UCF101 and OSCC, respectively. For a fair comparison, the frame-wise masking strategy adopts the same $\rho_{pre}$ of \textbf{EVEREST}.}
\begin{tabular}{lccc}
\hline
\multirow{2}{*}{PT-Making} & \multirow{2}{*}{FT-Masking}  & \multicolumn{2}{c}{Top-1}\\
&&{UCF101}&{OSCC}\\ \hline
% Random  & - & {87.9}  & {73.9}          \\
% Random  & Random & {84.9}  & {73.7}          \\ \hline
Frame-wise  & - & {68.5}  & {69.8}          \\
Frame-wise  & Frame-wise & {72.4}  & {69.2}          \\ \hline
\cellcolor{gg}\textbf{EVEREST}  & \cellcolor{gg}\textbf{EVEREST} & \cellcolor{gg}{89.7}  & \cellcolor{gg}{73.9}          \\ \hline
\end{tabular}
\end{table}

==> contents/table_mcs.tex <==
% \begin{table}[t!]
% \hfill
% \begin{minipage}{\linewidth}
%     \vspace{-0.1in}
%     \input{contents/table_oscc_results}
% \end{minipage}
%     \vspace{-0.05in}
%     \caption{\small \textbf{Comparison with public SoTA methods for OSCC on Ego4D val set.} We set the motion-centric sampling rate $\alpha=1.5$. Pre-trained data modalities from the OSCC dataset ‘V’ and ‘T’ refers to visual and text, respectively.}
%     \label{tab:table_mcs}
%     \vspace{-0.1in}
% \end{table}



% \begin{table}[t!]
% % \vspace{-0.15in}
% \begin{minipage}{0.26\linewidth}
%     \vspace{-0.1in}
%     \input{contents/table_mcs_ratio_1}
% \end{minipage}
% \hfill
% \begin{minipage}{0.73\linewidth}
%     \vspace{-0.1in}
%     \input{contents/table_oscc_results}
% \end{minipage}
%     \vspace{-0.05in}
%     \caption{\small \textbf{Effect of Motion-centric Sampling ratios ~(Left) and Comparison to public SoTA methods for OSCC on Ego4D val set~(Right).} We set the default motion-centric sampling rate ($\alpha=1.5$) and report fine-tuning accuracy. Pre-trained data modalities from the OSCC dataset ‘V’ and ‘T’ refers to visual and text.}
%     \label{tab:table_mcs}
%     \vspace{-0.1in}
% \end{table}

==> contents/table_mcs_ratio_1.tex <==
\vspace{0.05in}
\centering
        \resizebox{\textwidth}{!}{
        \renewcommand{\arraystretch}{0.95}
        \renewcommand{\tabcolsep}{2pt}
        \begin{tabular}{c c}
        \toprule
        \vspace{-0.02in}
        $\alpha$ & \textbf{Acc. (\%)} \\
        \midrule
        { -} & { 73.17}\\
        { 1.3} & { 73.54}\\
        \highlight{ 1.5} & { \textbf{73.85}}\\
        { 1.8} & { 73.79}\\
        { 2.0} & { 73.80}\\
\bottomrule
\end{tabular}}

==> contents/table_mcs_ratio_2.tex <==
\vspace{0.05in}
\centering
        \resizebox{\textwidth}{!}{
        \renewcommand{\arraystretch}{1.0}
        \renewcommand{\tabcolsep}{2pt}
        \begin{tabular}{c c}
        \toprule
        \vspace{-0.02in}
        $\alpha_{fine}$ & \textbf{Acc. (\%)} \\
        \midrule
        { -} & { 74.4}\\
        { 1.5} & { xx.x}\\
        { 2.0} & { xx.x}\\
        { 2.5} & { xx.x}\\
        { 3.0} & { xx.x}\\
\bottomrule
\end{tabular}}

==> contents/table_pt_ft_mem.tex <==
\begin{table}
  \begin{minipage}[t]{.48\textwidth}
    \caption{\small \textbf{Pre-training time \& Memory comparison with SoTA MVAs on K400.} We measure the pre-training time for an epoch under a single-node machine equipped with 8$\times$A6000~(48GB) GPUs. We use ViT-B and a batch size of 128. Note that MME~\citep{sun2023mme} should pre-compute the optical flow for the entire video data before pre-training. We exclude the time and memory of MME for optical flow computations in the table.}
  % \centering
    % \begin{adjustbox}{width=\columnwidth, center}
    \vspace{-0.1in}
    \scalebox{0.99}{
        \begin{tabular}{lcc}
        \hline
        Method                 & PT-Time & Memory \\ \hline
        VideoMAE~\citep{tong2022videomae}               & 18m   42s            & 150.3 GB              \\
        MME~\citep{sun2023mme}                    & 10m   15s            & 121.2 GB              \\
        MVD~\citep{wang2023mvd}                    & 51m   55s            & 274.9 GB              \\
        \cellcolor{gg}\textbf{EVEREST   (ours)} & \cellcolor{gg}\textbf{8m   18s}    & \cellcolor{gg}~\textbf{66.3} GB      \\ \hline
        \end{tabular}
    }
    \vspace{0.1in}
    % \end{adjustbox}
  \label{tab:pt_mem}%
  \end{minipage}%
  \hfill%
  \begin{minipage}[t]{.48\textwidth}
    \caption{\small \textbf{EVEREST-Finetuning with other MVAs on K400.} We apply our EVEREST for finetuning the pre-trained models~(ViT-B) by SoTA MVAs. We measure the memory usage with the same batch size of 128. While SoTA methods use full tokens during fine-tuning, our EVEREST uses only redundancy-robust tokens that \textbf{reduces significant computational cost and memory usage} with comparable accuracy.}
    \vspace{-0.1in}
    \scalebox{0.90}{
        \begin{tabular}{ccccc}
        \hline
        PT-Method & FT-Method       & GFLOPs & Memory  & Top-1         \\ \hline
        VideoMAE  & Full-token      & 180.5  & 362.5 GB      & 81.5          \\
        \cellcolor{gg}VideoMAE  & \cellcolor{gg}\textbf{EVEREST}   & \cellcolor{gg}98.1   & 1\cellcolor{gg}78.4 GB      & \cellcolor{gg}81.6          \\ \hline
        MME       & Full-token      & 180.5  & 362.5 GB      & 81.8          \\
        \cellcolor{gg}MME       & \cellcolor{gg}\textbf{EVEREST}   & \cellcolor{gg}98.1   & \cellcolor{gg}178.4 GB      & \cellcolor{gg}82.0          \\ \hline
        MVD       & Full-token      & 180.5  & 362.5 GB      & 83.4          \\
        \cellcolor{gg}MVD       & \cellcolor{gg}\textbf{EVEREST}   & \cellcolor{gg}98.1   & \cellcolor{gg}178.4 GB      & \cellcolor{gg}82.8          \\ \hline
        \end{tabular}
    }
    \label{tab:ft_mem}%
    \end{minipage}
  \vspace{-0.25in}
\end{table}


==> contents/table_pt_time_comparison.tex <==
\begin{table}[t]
\small
  \centering
\caption{\small \textbf{Pre-training time comparison with state-of-the-art MVMs.} We measure the pre-training time per epoch under the same single-node machine equipped with 8$\times$A6000~(48GB) GPUs. We use ViT-B as a backbone and a batch size of 128. Note that MME~\citep{sun2023mme} requires optical flow for its motion trajectory target, MME had to pre-compute the optical flow across the whole data before pre-training. So the measured pre-training time of MME does not include the computing time of optical flow~(refer to \href{https://github.com/XinyuSun/MME}{MME's official code}). }
\begin{tabular}{lcc}
\hline
Method                 & Time per epoch & Memory usage \\ \hline
VideoMAE~\citep{tong2022videomae}               & 18m   42s            & 150.3 GB              \\
MME~\citep{sun2023mme}                    & 10m   15s            & 121.2 GB              \\
MVD~\citep{wang2023mvd}                    & 51m   55s            & 274.9 GB              \\
\textbf{EVEREST   (ours)} & \textbf{8m   18s}    & ~\textbf{66.3} GB      \\ \hline
\end{tabular}
\end{table}


==> contents/table_resource.tex <==
\begin{wraptable}{r}{0.46\textwidth}
\centering
% \vspace{-0.1in}
\resizebox{0.98\linewidth}{!}{
\renewcommand{\arraystretch}{1.1}
\renewcommand{\tabcolsep}{3pt}
\begin{tabular}{ccccc}
\toprule
Effective Batch Size & 128 & 256 & 512 & 1024\\
\midrule
VideoMAE~\cite{tong2022videomae} & ~~258.4 GB~~ & ~~486.4 GB~~ & \emph{Out-of-Memory} & \emph{Out-of-Memory}\\
VideoMS (Ours) & ~~\textbf{60.0 GB}~~ & ~~\textbf{91.2 GB}~~ & ~~\textbf{151.2 GB}~~ & ~~\textbf{273.6 GB}~~\\
\bottomrule
\end{tabular}}
\vspace{-0.05in}
% \caption{\small Memory allocation comparison using ViT-B in the pre-training phase using one node with A100$\times$8 GPUs. VideoMAE suffers from the \emph{Out-Of-Memory} issue when using a batch size larger than 256.}
\caption{\small Memory allocation comparison using ViT-B in the pre-training phase (one node, A100$\times$8 GPUs). VideoMAE suffers from \emph{Out-Of-Memory} issue when the batch size is larger than 256.}
\label{tab:mem-allocation}
\vspace{-0.1in}
\end{wraptable}

==> contents/table_resource2.tex <==
\begin{table}[t!]
% \vspace{0.05in}
\centering
\caption{\small \textbf{Memory allocation comparison} in the pre-training phase (one node, A100$\times$8 GPUs). The memory gaps grow up when increasing batch size and model size. Especially our MATS with ViT-L (164.1GB) achieves about 4 times better efficiency than VideoMAE (634.1GB).}
% \begin{adjustbox}{width=\columnwidth, center}
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{lccccc}
\toprule
    \multirow{2}{*}{Method} & \multirow{2}{*}{Backbone} & \multicolumn{4}{c}{Effective Batch Size}\\
    && 128 & 256 & 512 & 1024\\
\midrule
&{ViT-S} & ~~71.9 GB~~ & ~~117.4 GB~~ & ~~233.6 GB~~ & ~~443.6 GB~~ \\
VideoMAE~\cite{tong2022videomae}&{ViT-B} & ~~258.4 GB~~ & ~~486.4 GB~~ & \emph{Out-of-Memory} & \emph{Out-of-Memory}\\
&{ViT-L} & ~~353.9 GB~~ & ~~634.1 GB~~ & \emph{Out-of-Memory} & \emph{Out-of-Memory}\\
\midrule
 &{ViT-S}& ~~\textbf{31.9 GB}~~ & ~~\textbf{59.9 GB}~~ & ~~\textbf{95.6 GB}~~ & ~~\textbf{173.1 GB}~~\\
MATS (Ours) &{ViT-B}& ~~\textbf{60.0 GB}~~ & ~~\textbf{91.2 GB}~~ & ~~\textbf{151.2 GB}~~ & ~~\textbf{273.6 GB}~~\\
 &{ViT-L}& ~~\textbf{117.3 GB}~~ & ~~\textbf{164.1 GB}~~ & ~~\textbf{258.9 GB}~~ & ~~\textbf{428.4 GB}~~\\
\bottomrule
\end{tabular}}
% \end{adjustbox}
\label{tab:mem-allocation2}
% \vspace{-0.15in}
\end{table}
% \begin{table}[t!]
% % \vspace{0.05in}
% \centering
% \caption{\small Memory allocation comparison in the pre-training phase (one node, A100$\times$8 GPUs). The memory gaps grow up when increasing batch size and model size. Especially our MATS with ViT-L (164.1GB) achieves about 4 times better efficiency than VideoMAE (634.1GB).}
% % \begin{adjustbox}{width=\columnwidth, center}
% \resizebox{0.4\linewidth}{!}{
% \begin{tabular}{lccccc}
% \toprule
%     \multirow{2}{*}{Method} & \multirow{2}{*}{Backbone} & \multicolumn{4}{c}{Effective Batch Size}\\
%     && 128 & 256 & 512 & 1024\\
% \midrule
% &{ViT-S} & 71.9  & 117.4  & 233.6  & 443.6  \\
% VideoMAE&{ViT-B} & 258.4  & 486.4  & \emph{OOM} & \emph{OOM}\\
% &{ViT-L} & 353.9  & 634.1  & \emph{OOM} & \emph{OOM}\\
% \midrule
%  &{ViT-S}& \textbf{31.9 } & \textbf{59.9 } & \textbf{95.6 } & \textbf{173.1 }\\
% Ours &{ViT-B}& \textbf{60.0 } & \textbf{91.2 } & \textbf{151.2 } & \textbf{273.6 }\\
%  &{ViT-L}& \textbf{117.3 } & \textbf{164.1 } & \textbf{258.9 } & \textbf{428.4 }\\
% \bottomrule
% \end{tabular}}
% % \end{adjustbox}
% \label{tab:mem-allocation2}
% % \vspace{-0.15in}
% \end{table}

==> contents/table_small_dataset.tex <==
\begin{table}[t!]
% \vspace{0.05in}
\centering
\caption{\small \textbf{Performance comparison with strong baselines on UCF101, HMDB51, SSv2, and Kinetics-400 datasets}. Several results are drawn from \cite{diba2021vi2clr} and \cite{tong2022videomae}.}
\begin{adjustbox}{width=\columnwidth, center}
% \resizebox{0.9\linewidth}{!}{
% \renewcommand{\arraystretch}{1.2}
% \renewcommand{\tabcolsep}{3pt}
\begin{tabular}{l c c c c c c c c c}
\toprule
    \multirow{2}{*}{Method} & \multirow{2}{*}{Backbone} & \multirow{2}{*}{Pre-train Data} & \multirow{2}{*}{Frames} & UCF101&HMDB51&\multicolumn{2}{c}{SSv2}&\multicolumn{2}{c}{Kinetics-400} \\
    &&&&{T1}&{T1} &T1&T5&T1&T5\\
\midrule
    % OPN \cite{lee2017unsupervised}& {VGG} & {UCF101} & {N/A} & {59.6} & {23.8}\\
    VCOP~\cite{xu2019self}& {R(2+1)D} & {UCF101} & {N/A} & {72.4} & {30.9} &{N/A}&{N/A}&{N/A}&{N/A}\\
    CoCLR~\cite{han2020self}& {S3D-G} & {UCF101} & {32} & {81.4} & {52.1} &{N/A}&{N/A}&{N/A}&{N/A}\\
    Vi$^{2}$~CLR\cite{diba2021vi2clr}& {S3D} & {UCF101} & {32} & {82.8} & {52.9} &{N/A}&{N/A}&{N/A}&{N/A}\\
    CoCLR~\cite{han2020self}& {S3D-G} & {K400} & {32} & {87.9} & {54.6} &{N/A}&{N/A}&{N/A}&{N/A}\\
    Vi$^{2}$~CLR\cite{diba2021vi2clr}& {S3D} & {K400} & {32} & {89.1} & {55.7} &{N/A}&{N/A}&{71.2}&{N/A}\\
    RSPNet~\cite{chen2021rspnet}& {S3D-G} & {K400} & {64} & {93.7} & {64.7} &{55.0}&{N/A}&{N/A}&{N/A}\\    
    % $\rho\text{SimCLR}_{\rho=2}${\scriptsize \cite{feichtenhofer2021large}}& {SlowOnly-R50} & {K400} & {8} & {88.9} & {N/A} \\    
    $\rho\text{SwAV}_{\rho=2}$~{\cite{feichtenhofer2021large}}& {SlowOnly-R50} & {K400} & {8} & {87.3} & {N/A}&{N/A}&{N/A}&{61.6}&{N/A}\\
    $\rho\text{MoCo}_{\rho=2}$~{\cite{feichtenhofer2021large}}& {SlowOnly-R50} & {K400} & {8} & {91.0} & {N/A}&{N/A}&{N/A}&{65.8}&{N/A}\\
    $\rho\text{BYOL}_{\rho=2}$~{\cite{feichtenhofer2021large}}& {SlowOnly-R50} & {K400} & {8} & {92.7} & {N/A}&{N/A}&{N/A}&{65.8}&{N/A}\\
    VideoMAE~\cite{tong2022videomae}&{ViT-B}&{UCF101 / HMDB51}&{16} &{91.3} & {62.6}&{N/A}&{N/A}&{N/A}&{N/A}\\
\midrule
    \textbf{MATS (Ours)}&{ViT-B}&{UCF101 / HMDB51}&{16}&{93.4} & {68.1}&{N/A}&{N/A}&{N/A}&{N/A}\\
    % VIMPAC\cite{tan2021vimpac}& {S-T transformer} & {HowTo100M} & {10} & {92.7} & {65.9} \\
\midrule
    VideoMAE~\cite{tong2022videomae}&{ViT-S}&{K400}&{16} &{N/A} & {N/A}&{N/A}&{N/A}&{79.0}&{93.8}\\
    VideoMAE~\cite{tong2022videomae}&{ViT-B}&{K400}&{16} &{96.1} & {73.3}&{69.7}&{92.3}&{81.5}&{95.1}\\
    VideoMAE~\cite{tong2022videomae}&{ViT-L}&{K400}&{16} &{N/A} & {N/A}&{74.0}&{94.6}&{85.2}&{96.8}\\
    VideoMAE~\cite{tong2022videomae}&{ViT-S}&{SSv2}&{16} &{N/A} & {N/A}&{66.8}&{90.3}&{N/A}&{N/A}\\
    VideoMAE~\cite{tong2022videomae}&{ViT-B}&{SSv2}&{16} &{N/A} & {N/A}&{70.8}&{92.4}&{N/A}&{N/A}\\
    VideoMAE~\cite{tong2022videomae}&{ViT-L}&{SSv2}&{16} &{N/A} & {N/A}&{74.3}&{94.6}&{N/A}&{N/A}\\
\midrule
    \textbf{MATS (Ours)}&{ViT-S}&{SSv2 / K400}& {16} &{N/A} & {N/A}&&&&\\
    \textbf{MATS (Ours)}&{ViT-B}&{SSv2 / K400}&{16}&{N/A} & {N/A}&&&&\\
    \textbf{MATS (Ours)}&{ViT-L}&{SSv2 / K400}&{16} &{N/A} & {N/A}&&&&\\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:main}
% \vspace{-0.15in}
\end{table}

==> contents/table_ssv2.tex <==
% \begin{table*}[t]
% \caption{\small Results of transferable robustness in 5-way 5-shot unseen domain tasks that are trained on 5-way 5-shot CIFAR-FS. Rob. stands for accuracy(\%) that is calculated with PGD-20 attack ($\epsilon=8./255.$, step size=$\epsilon/10$). Clean stands for test accuracy(\%) of clean images. All models are trained with PGD-7 attacks on ResNet12.}
% \centering
% \vspace{0.1in}
% \begin{adjustbox}{width=0.9\textwidth}
%     \begin{tabular}{lcccccccccc} %Resnet12, attack7
%     \toprule
%     &\multicolumn{10}{c}{CIFAR-FS $\rightarrow$}\\
%     & \multicolumn{2}{c}{Mini-ImageNet}& \multicolumn{2}{c}{Tiered-ImageNet}&\multicolumn{2}{c}{CUB}&\multicolumn{2}{c}{Flowers}& \multicolumn{2}{c}{Cars}\\
%     \cmidrule(r){2-11}
%     & Clean & Rob.& Clean & Rob.& Clean & Rob. &Clean& Rob.&Clean& Rob.\\
%     \midrule
%     MAML~\citep{finn2017model} & \underline{44.85}&6.21& \textbf{61.19}&2.48&\underline{48.41}&3.46&\textbf{67.76}&5.73&\textbf{43.94}&5.31 \\
%     ADML~\citep{yin2018adml} & 28.66&6.53&40.06&\underline{11.36}&31.18&5.21&39.36&\underline{11.26}&27.43&3.18\\
    
%     AQ~\citep{goldblum2020adversarially}&33.09&3.32&37.41&5.05&38.37&4.10&60.14&11.03&36.83&4.47\\
%     % AQ r2d2
%     %AQ~\citep{goldblum2020adversarially}&36.46&16.10&41.89&21.78&50.97&20.78&75.33&43.36&45.85&20.02\\
%     RMAML~\citep{wang2021rmaml}&28.05& \underline{6.65}&29.54&9.30&30.24&\underline{5.67}&42.91&10.79&31.72&\underline{5.56}\\
%     Ours&\textbf{45.82}&\textbf{24.12}&	 \underline{51.46}&\textbf{30.06}&\textbf{48.56}&	\textbf{25.23}&\underline{66.49}&\textbf{42.16}&	 \underline{38.29}&\textbf{19.43}\\
%     \bottomrule
%     \end{tabular}
%     \label{table:cifar-crossdomain}
% \vspace{-1.4in}
% \end{adjustbox}
% \end{table*}


\begin{table*}[t!]
\vspace{0.05in}
\centering
\resizebox{1.0\linewidth}{!}{
\renewcommand{\arraystretch}{1.2}
\renewcommand{\tabcolsep}{3pt}
\begin{tabular}{l c c c c c}
\toprule
    {Method} & {Backbone} & {Pre-train data} & {Frames} & {GFLOPs} & {Top-1 Acc.(\%)} \\
\midrule
    $\text{TEINet}_{\emph{En}}$ \citep{liu2020teinet}&{ResNet50}_{\times2}&{ImageNet-1K}&{8+16}&99\times10\times3&66.5\\
    $\text{TANet}_\emph{En}$~\cite{liu2021tam}&{ResNet50}_{\times2}&{ImageNet-1K}&{8+16}&99\times2\times3&66.0\\
    $\text{TDN}_\emph{En}$~\cite{wang2021tdn}&{ResNet101}_{\times2}&{ImageNet-1K}&{8+16}&198\times1\times3&69.6\\
    SlowFast~\cite{feichtenhofer2019slowfast}&{ResNet101}&{K400}&{8+32}&106\times1\times3&63.1\\
    MViTv1~\cite{fan2021multiscale}&{MViTv1-B}&{K400}&{64}&455\times1\times3&67.7\\
    TimeSformer~\cite{bertasius2021timesformer}&{ViT-B}&{ImageNet-21K}&{8}&196\times1\times3&59.5\\
    TimeSformer~\cite{bertasius2021timesformer}&{ViT-L}&{ImageNet-21K}&{64}&5549\times1\times3&62.4\\
    ViViT FE~\cite{arnab2021vivit}&{ViT-L}&{ImageNet-21K+K400}&{32}&995\times4\times3&65.9\\
    Motionfromer~\cite{patrick2021mformer}&{ViT-B}&{ImageNet-21K+K400}&{16}&370\times1\times3&66.5\\    
    Motionfromer~\cite{patrick2021mformer}&{ViT-L}&{ImageNet-21K+K400}&{32}&1185\times1\times3&68.1\\    
    Video Swin~\cite{liu2022videoswin}&{Swin-B}&{ImageNet-21K+K400}&{32}&321\times1\times3&69.6\\    
    VIMPAC~\cite{tan2021vimpac}&{ViT-L}&{HowTo100M+DALLE}&{10}&N/A\times10\times3&68.1\\    
    BEVT~\cite{wang2022bevt}&{Swin-B}&{ImageNet-1K+K400+DALLE}&{32}&321\times1\times3&70.6\\    
    MaskFeat~\cite{wang2022bevt}&{MViT-L}&{K600}&{40}&2828\times1\times3&75.0\\    
    VideoMAE~\cite{tong2022videomae}&{ViT-B}&{K400}&{16}&180\times2\times3&69.7\\    
    VideoMAE~\cite{tong2022videomae}&{ViT-L}&{K400}&{16}&597\times2\times3&74.0\\    
    VideoMAE~\cite{tong2022videomae}&{ViT-S}&{SSv2}&{16}&180\times2\times3&66.8\\    
    VideoMAE~\cite{tong2022videomae}&{ViT-B}&{SSv2}&{16}&180\times2\times3&70.8\\    
    VideoMAE~\cite{tong2022videomae}&{ViT-L}&{SSv2}&{16}&597\times2\times3&74.3\\    
    VideoMAE~\cite{tong2022videomae}&{ViT-L}&{SSv2}&{32}&1436\times2\times3&75.4\\        
    MAE~\cite{feichtenhofer2022masked}&{ViT-L}&{K400}&{16}&598\times1\times3&72.1\\        
    MAE~\cite{feichtenhofer2022masked}&{ViT-H}&{K400}&{16}&1193\times1\times3&74.1\\        
    MAE~\cite{feichtenhofer2022masked}&{ViT-L}&{K600}&{16}&598\times1\times3&73.0\\        
    MAE~\cite{feichtenhofer2022masked}&{ViT-H}&{K600}&{16}&1193\times1\times3&75.2\\        
    MAE~\cite{feichtenhofer2022masked}&{ViT-L}&{K700}&{16}&598\times1\times3&73.6\\        
    MAE~\cite{feichtenhofer2022masked}&{ViT-H}&{K700}&{16}&1193\times1\times3&75.5\\        
    % MaskFeat~\cite{wang2022bevt}&{MViT-L}&{K600}&{40}&2828\times1\times3&75.0\\    
    % MaskFeat~\cite{wang2022bevt}&{MViT-L}&{K600}&{40}&2828\times1\times3&75.0\\    
    % MaskFeat~\cite{wang2022bevt}&{MViT-L}&{K600}&{40}&2828\times1\times3&75.0\\    
\midrule
    \textbf{VideoMS(Ours)}&{ViT-B}&{SSv2}&{16}&138\times2\times3&\textbf{75.4}\\
\bottomrule
\end{tabular}}
\vspace{-0.05in}
\caption{\small \textbf{Comparison to state-of-the-art methods on UCF101 and HMDB51.} We outperform the previous method, including the masking-based video model, without using the pre-training step on a large-scale dataset. These results are drawn from \cite{diba2021vi2clr} and \cite{tong2022videomae}.}
\label{tab:table_ssv2}
\vspace{-0.1in}
\end{table*}

==> contents/table_ucf_hmdb.tex <==
\begin{table}[t]
% \vspace{0.05in}
\centering
\caption{\small \textbf{Performance comparison with strong baselines on
UCF101 and HMDB51 datasets} without using the pre-training step on a large-scale dataset. Several results are drawn from \cite{diba2021vi2clr} and \cite{tong2022videomae}.}
% \begin{adjustbox}{width=\columnwidth, center}
\resizebox{0.7\columnwidth}{!}{
    % \renewcommand{\arraystretch}{1.0}
    % \renewcommand{\tabcolsep}{3pt}
\begin{tabular}{l c c c c c}
\toprule
    \multirow{2}{*}{Method} & \multirow{2}{*}{Backbone} & \multirow{2}{*}{Extra data} & \multirow{2}{*}{Frames} & \multicolumn{2}{c}{Top-1 Acc.(\%)}\\
    &&&&{\textbf{UCF101}}&{\textbf{HMDB51}}\\
\midrule
    % OPN \cite{lee2017unsupervised}& {VGG} & {UCF101} & {N/A} & {59.6} & {23.8}\\
    VCOP~\cite{xu2019self}& {R(2+1)D} & {UCF101} & {N/A} & {72.4} & {30.9}\\
    CoCLR~\cite{han2020self}& {S3D-G} & {UCF101} & {32} & {81.4} & {52.1}\\
    Vi$^{2}$~CLR\cite{diba2021vi2clr}& {S3D} & {UCF101} & {32} & {82.8} & {52.9}\\
    CoCLR~\cite{han2020self}& {S3D-G} & {K400} & {32} & {87.9} & {54.6}\\
    Vi$^{2}$~CLR\cite{diba2021vi2clr}& {S3D} & {K400} & {32} & {89.1} & {55.7}\\
    RSPNet~\cite{chen2021rspnet}& {S3D-G} & {K400} & {64} & {93.7} & {64.7}\\    
    % $\rho\text{SimCLR}_{\rho=2}${\scriptsize \cite{feichtenhofer2021large}}& {SlowOnly-R50} & {K400} & {8} & {88.9} & {N/A} \\    
    $\rho\text{SwAV}_{\rho=2}$~{\cite{feichtenhofer2021large}}& {SlowOnly-R50} & {K400} & {8} & {87.3} & {N/A}\\
    $\rho\text{MoCo}_{\rho=2}$~{\cite{feichtenhofer2021large}}& {SlowOnly-R50} & {K400} & {8} & {91.0} & {N/A}\\
    $\rho\text{BYOL}_{\rho=2}$~{\cite{feichtenhofer2021large}}& {SlowOnly-R50} & {K400} & {8} & {92.7} & {N/A}\\
\midrule    
    VideoMAE~\cite{tong2022videomae}&{ViT-B}&{\ding{55}}&{16} &{91.3} & {62.6}\\
\midrule
    \textbf{MATS (Ours)}&{ViT-B}&{\ding{55}}&{16}&{93.4} & {68.1}\\
\bottomrule
\end{tabular}}
% \end{adjustbox}
\label{tab:ucf&hmdb}
% \vspace{-0.15in}
\end{table}

==> defs.tex <==

%\usepackage[numbers, sort&compress]{natbib}

\usepackage{pifont}
\usepackage{amsmath, amssymb, bm, amsthm}
\usepackage{mathrsfs} 
\usepackage{mathtools}
\usepackage{thmtools}
\usepackage{enumitem}
\usepackage{subfigure}
\usepackage{color}
\usepackage{booktabs}
\usepackage{array}
\usepackage{tabularx, booktabs, multirow}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}

%\usepackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}


\usepackage[capitalize,nameinlink]{cleveref}


%\numberwithin{equation}{section}
%\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
%\newtheorem{defn}{Definition}[section]
\newtheorem{lem}{Lemma}[section]
%\newtheorem{cor}{Corollary}[section]
\newtheorem{cor}{Corollary}
%\newtheorem{prop}{Proposition}[section]
%\theoremstyle{definition}
%\newtheorem{algorithm}{Algorithm}[section]
%\newtheorem{example}{Example}[section]


\newcommand{\dee}{\mathrm{d}}
\newcommand{\grad}{\nabla}

\DeclareMathOperator{\ber}{Ber}
\DeclareMathOperator{\gammadist}{Gamma}
\DeclareMathOperator{\betadist}{Beta}
\DeclareMathOperator{\dir}{Dir}
%\DeclareMathOperator{\cat}{cat}
\DeclareMathOperator{\expon}{expon}
%\DeclareMathOperator{\unif}{unif}
%\DeclareMathOperator{\KL}{KL}
\DeclareMathOperator{\sgm}{sgm}
\DeclareMathOperator{\frob}{{F}}
\DeclareMathOperator{\softmax}{{softmax}}
\DeclareMathOperator{\var}{{Var}}
\DeclareMathOperator{\diag}{{diag}}
\DeclareMathOperator{\softplus}{{Softplus}}
\DeclareMathOperator{\pool}{{StatisticsPooling}}

\newcommand{\normal}{\mathcal{N}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\card}[1]{\vert {#1} \vert}
\newcommand{\distiid}{\overset{iid}{\dist}}
\newcommand{\distind}{\overset{ind}{\dist}}
\newcommand{\Indicator}[1]{\mathds{1}_{\{#1\}}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\defas}{\vcentcolon=}  % requires mathtools package
\newcommand{\iid}{i.i.d.}

\newcommand{\bepsilon}{{\boldsymbol{\epsilon}}}
\newcommand{\btheta}{{\boldsymbol{\theta}}}
\newcommand{\bTheta}{{\boldsymbol{\Theta}}}
\newcommand{\bbeta}{{\boldsymbol{\beta}}}
%%\newcommand{\E}{{\mathbb{E}}}
\newcommand{\Real}{{\mathbb{R}}}
\newcommand{\calP}{{\mathcal{P}}}
\newtheorem{observation}{Observation}

\newcommand{\bzero}{\mathbf{0}}
\newcommand{\bone}{\mathbf{1}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bof}{\mathbf{f}}
\newcommand{\bhy}{\widehat{\by}}
%\newcommand{\bW}{\mathbf{W}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bh}{\mathbf{h}}
\newcommand{\bhW}{{\widehat{\bW}}}
\newcommand{\btW}{{\widetilde{\bW}}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bphi}{{\boldsymbol{\phi}}}
\newcommand{\bpi}{{\boldsymbol{\pi}}}
\newcommand{\noise}{{\boldsymbol{\varepsilon}}}

\newcommand{\ts}{{\tau}}

\newcommand{\bee}{\begin{eqnarray}}
\newcommand{\eee}{\end{eqnarray}}



==> figures/exp_results.tex <==
\begin{figure*}
    \small
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{cc}
    \includegraphics[height=6cm, width=7cm]{pre_results.pdf}&
     \includegraphics[height=6cm, width=7cm]{fine_results.pdf}\\
     (a) &
     (b) \\
    \end{tabular}}
     \caption{\footnotesize {\textbf{The Kinetics-400 performance comparison of masking-based approaches depends on the pre-training epochs and GFLOPs for fine-tuning.} }}
    \label{fig:exp_results}
\end{figure*}


==> figures/fig_analysis_1.tex <==
\begin{figure}[t]
    \centering
    \begin{tabular}{c}
        \includegraphics[width=0.32\textwidth]{figures/images/f1.png}\\
    \end{tabular}{c}
    \caption{\textbf{Performance comparison of contrastive and non-contrastive learning based approaches depending on the data size in local data.}}
    \label{fig:analysis_1}
\end{figure}

==> figures/flop_plot.tex <==
\begin{wrapfigure}{l}{0.48\textwidth}
\centering
    % \vspace{-0.05in}
    % \includegraphics[width=0.98\linewidth]{figures/images/pt_mem.pdf}\\
    \includegraphics[width=0.98\linewidth]{figures/images/flop_plot.pdf}\\
    \vspace{-0.1in}
    \caption{\small \textbf{Computation~(GFLOPs) comparison scaling ViT Backbones on Kinetics-400.}
    We compute GFLOPs during both pre-training and finetuning with batch size 1. Our MATS drastically reduce computation cost for all ViT backbones. We train both our MATS and VideoMAE~\cite{tong2022videomae} for 200 epochs.  
    }
    \label{fig:flop_plot}
    % \vspace{-0.1in}
\end{wrapfigure} 

==> figures/patch_embed.tex <==
\begin{figure}[t]
    \centering
    \begin{tabular}{c}
        \includegraphics[width=1.0\columnwidth]{figures/images/patch_embed.pdf}\\
    \end{tabular}
    \caption{\textbf{Illustration of tokenization and patch embedding layer.} }
    \label{fig:patch_embed}
\end{figure}

==> figures/plots.tex <==
\begin{wrapfigure}{o}{0.46\textwidth}
\centering
    % \vspace{-0.05in}
    \includegraphics[width=0.98\linewidth]{figures/images/merge_fig_3.pdf}\\
    \vspace{-0.1in}
    \caption{\small \textbf{Performance and efficiency of our MATS}. \textbf{(Left)} MATS outperforms the SoTA model (VideoMAE~\cite{tong2022videomae}) over UCF101, even at fewer training epochs. We additionally report the results of VideoMAE with a lower masking ratio (75\%) during pre-training. \textbf{(Right)} Our MATS drastically reduces GFLOPs during pre-training and fine-tuning compared to VideoMAE and MAE~\cite{feichtenhofer2022masked}.}
    \label{fig:a}
    % \vspace{-0.1in}
\end{wrapfigure} 

==> figures/pt_mem.tex <==
\begin{wrapfigure}{r}{0.46\textwidth}
\centering
    % \vspace{-0.05in}
    % \includegraphics[width=0.98\linewidth]{figures/images/pt_mem.pdf}\\
    \includegraphics[width=0.98\linewidth]{figures/images/pt_mem_annotated.pdf}\\
    \vspace{-0.1in}
    \caption{\small \textbf{Memory comparison with different batch sizes during pre-training phase.} 
    % Compared to VideoMAE~\cite{tong2022videomae} with ViT-L using 256 batch size, our MATS achives $\times 4$ better memory efficiency. 
    We measure the memory consumption using one node equipped with 8$\times$ A100~(80GB). VideoMAE~\cite{tong2022videomae} with ViT-B and ViT-L show \textit{out-of-memory} when using batch sizes of 256 and 512, respectively.
    Our MATS drastically reduces memory consumption with all ViT backbones and in particular, the memory usage gap gets bigger when using large model. \textit{e.g.}, MATS achieves $4 \times$ better efficiency than VideoMAE~\cite{tong2022videomae} with ViT-L using 256 batch size.  
    }
    \label{fig:pt_mem}
    % \vspace{-0.1in}
\end{wrapfigure} 

==> math_definition.tex <==
%%% load AMS-Latex Package
\usepackage{amsmath,amsfonts}
\usepackage{amsthm}
\usepackage{amssymb,amsopn}
\usepackage{bm} % bold symbol

\usepackage{graphicx}  %Required

% define fonts
\newcommand{\mbf}[1]{\mathbf{#1}} % vector, matrix
\newcommand{\bs}[1]{\boldsymbol{#1}} % boldsymbol

% define prob. dist. or func.
\newcommand{\bern}{\operatorname{ber}}
\newcommand{\kumar}{\operatorname{kumar}}
\newcommand{\sigm}{\operatorname{sgm}}
\newcommand{\unif}{\operatorname{unif}}
\newcommand{\kl}{\operatorname{KL}}
\newcommand{\cat}{\operatorname{cat}}
\newcommand{\nn}{\operatorname{NN}}

%%%% Special math symbols
\newcommand{\field}[1]{\mathbb{#1}}
\newcommand{\R}{\field{R}} % real domain
%\newcommand{\C}{\field{C}} % complex domain
\newcommand{\F}{\field{F}} % functional domain
%\newcommand{\T}{^{\top}\!\!} % transpose
%\newcommand{\T}{^{\textrm T}} % transpose
\newcommand{\TN}{^{-\textrm T}} % transpose
%\newcommand{\T}{^{\mathsf{T}}} % transpose


%%% define constant
\newcommand{\cst}[1]{\mathsf{#1}}

%% operator in linear algebra, functional analysis
\newcommand{\inner}[2]{#1\cdot #2}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\twonorm}[1]{\|#1\|_2^2}
% operator in functios, maps such as M: domain1 --> domain 2
\newcommand{\Map}[1]{\mathcal{#1}}

% operator in probability: expectation, covariance,
\newcommand{\ProbOpr}[1]{\mathbb{#1}}
% independence
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
% conditional independence
\newcommand{\cind}[3]{{#1} \independent{#2}\,|\,#3}
% conditional expectation
\newcommand{\cndexp}[2]{\ProbOpr{E}\,[ #1\,|\,#2\,]}

\def\D{\mathcal{D}}
\def\loss{\mathcal{L}}
\def\R{\mathcal{R}}
\def\real{\mathbb{R}}
\def\S{\mathcal{S}}

\def\U{\mathcal{U}}
\def\T{\mathsf{T}}

\newcommand\innerP[2]{\langle #1, \, #2 \rangle}
%\newcommand\biginner[2]{\big\langle #1, \, #2 \big\rangle}


% operator in optimization
\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator{\argmin}{arg\,min}
\newcommand{\todo}[1]{{\color{red}#1}}

\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\st}{s.t.}
\newcommand{\argmin}{\operatornamewithlimits{argmin}}

\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{remarks}{Remark}
\newtheorem{example}{Example}
\newtheorem{cond}{Condition}

\newlength{\widebarargwidth}
\newlength{\widebarargheight}
\newlength{\widebarargdepth}
\DeclareRobustCommand{\widebar}[1]{%
  \settowidth{\widebarargwidth}{\ensuremath{#1}}%
  \settoheight{\widebarargheight}{\ensuremath{#1}}%
  \settodepth{\widebarargdepth}{\ensuremath{#1}}%
  \addtolength{\widebarargwidth}{-0.3\widebarargheight}%
  \addtolength{\widebarargwidth}{-0.3\widebarargdepth}%
  \makebox[0pt][l]{\hspace{0.15\widebarargheight}%
    \hspace{0.3\widebarargdepth}%
    \addtolength{\widebarargheight}{0.3ex}%
    \rule[\widebarargheight]{0.95\widebarargwidth}{0.1ex}}%
  {#1}}



\newcommand{\eat}[1]{}


\DeclareMathOperator{\KL}{KL}
\newcommand{\E}{\mathbb{E}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\retain}{\rho}
\newcommand{\bsretain}{\boldsymbol{\rho}}
\newcommand{\indc}[1]{\mathbb{I}_{\{#1\}}}
\newcommand{\bnu}{{\bs\nu}}
\newcommand{\pout}{{p_{\texttt{out}}}}
\newcommand{\qin}{{q_{\texttt{in}}}}
\newcommand{\qout}{{q_{\texttt{out}}}}
\newcommand{\bbX}{{\mathcal{X}}}
\newcommand{\bbY}{{\mathcal{Y}}}
